A Holistic Approach for Soundness Verification of Decision-Aware Process Models (extended version)

The last decade has witnessed an increasing transformation in the design, engineering, and mining of processes, moving from a pure control-flow perspective to more integrated models where also data and decisions are explicitly considered. This calls for methods and techniques able to ascertain the correctness of such integrated models. Differently from previous approaches, which mainly focused on the local interplay between decisions and their corresponding outgoing branches, we introduce a holistic approach to verify the end-to-end soundness of a Petri net-based process model, enriched with case data and decisions. In particular, we present an effective, implemented technique that verifies soundness by translating the input net into a colored Petri net with bounded color domains, which can then be analyzed using conventional tools. We prove correctness and termination of this technique. In addition, we relate our contribution to recent results on decision-aware soundness, showing that our approach can be readily applied there.

==> discussion-technical.tex <==
\subsection{Optimizations}
\marco{Brevissima discussione su modi di ottimizzare la costruzione del reachability graph, spingendo in avanti il nondeterminismo}.


\subsection{Extensions of the Model}
\marco{Possibili estensioni che intendiamo studiare. Prova di indecidibilita su Z con +1 per mostrare che non si puo fare molto su domini piu ricchi.}


==> representative-nets.tex <==
\section{Representative nets}


Clearly, the major difficulty is that a direct and exhaustive computation is not viable, because $\Universe$ is in general infinite as it is also any domain $\Domain$ associated to any variable $\var$, and thus the set of possible values $\varState(\var)$ considered at any point (including the initial one). 
%%

Our approach is based on a translation of DPN-nets into CPNs so that, in addition to providing a feasible solution to the problem, we also make standard techniques and tools for characterising and analysing the reachability graph available off-the-shelf.

We start by tackling the infiniteness of the possible values for each variable, relying on the notion of representatives of infinite intervals defined as equivalence classes with respect to the process at hand. The intuition is as follows: instead of enumerating one by one the possible values, we group them into classes that have the property that the specific DPN-net is not able to distinguish values belonging to the same class, so that we can  pick arbitrarily a representative for the entire class and reason only with it. We are going to show how the number of such classes is finite, and also known in advance. 

\begin{definition}[Normal form]
\paolo{la scrivero' ma non serve per poter continuare, al momento}
\end{definition}

From now on, we will only consider DPN-nets in normal form. 

\begin{definition}[Constants of the process]
The set of \emph{constants} related to a variable $\var\in\Vars$ of a DPN-net is the set $\Consts{\var}\subset\varDomain$ that is the union of:
\begin{compactitem}
\item the set of all the values $k$ such that $\var \odot k$ appears in any guard of any $t\in T$;
\item special values $\infty$ (resp. $-\infty$) if $\varDomain$ does not have a maximal (resp. minimal) element.\paolo{in questo modo però li prendo anche come rappresentati.. ma servono per definire $\Repres{\var}$. Da migliorare...}
\end{compactitem}
\end{definition}



Observing that each such set $\Consts{\var}$ is finite and ordered, for each of these  we partition the universe $\Universe$ into $\card{\Consts{\var}}-1$ equivalence classes, corresponding to intervals of values in which $\Universe$ can be partitioned wrt $\var$, and for each elect a \emph{representative} as follows: 
\[ 
\Repres{\var}:=\{ x\in\varDomain \mid x\in \Consts{\var} \text{ or } x= pick(x_1,x_2) \text{ for consecutive } x_1,x_2\in\Consts{\var}\}
\]

\noindent 
where $pick$ returns an arbitrary representatives value in the specified interval that is also in $\varDomain$, excluding the endpoints\footnote{for dense domains such as real numbers such intervals are always nonempty, whereas for non-dense domains they might be so. In this case, we consider $pick$ undefined, so that no representative is added to $\Repres{\var}$ for empty intervals.}. For a given value $x$ in the original domain $\varDomain$, we denote its representative as $rep(x)$, namely $rep(x):=x$ iff $x\in \Consts{\var}$, otherwise $rep(x)=y$ implies both $y\in(x_1,x_2)$ and $x\in(x_1,x_2)$. For $\bot$, we define $rep(\bot):=\bot$.

 Let $\Repres{} := \set{\Repres{{\var}_1},\ldots, \Repres{{\var}_q}}$ for each variable ${\var}_i\in\Vars$. We define a variable assignment \emph{restricted to} $\Repres{}$ as a function $\varStateR : \Vars \rightarrow \cup_{\var}\Repres{\var}$, with the restriction that $\varStateR(\var)\in  \Repres{\var}$ for any $\var$. 
%%
Given a variable assignment $\varState$ on the original domain $\varDomain$ of each variable $\var\in\Vars$, we \emph{compute} its restriction as: 
%%
\[
\restrict{\varState}(\var) := rep(\varState(\var)).
\]

\begin{definition}[Representative net]
Given a DPN-net $N$ and the set $\Repres{}$ for $N$ as above, we define the \emph{representative net} $N_{\Repres{}}$ as the DPN-net computed as follows:
\begin{compactitem}
\item $(P,T,F)$ is as in $N$;
\item the set $\Vars$ is as in $N$, but for each variable name $v\in \VarNames$ we \emph{redefine} the domain of the corresponding typed variable $\var$ with $\Domain := \tup{\Repres{\var},\Preds}$;
\item $\varState_I$ is replaced with $\restrict{\varState_I}$;
\item $\writes$ and $\guard$ are as in $N$. 
\end{compactitem}
\end{definition}

As a result, the new states of $N_{\Repres{}}$ as of the form $(M,\varStateR{})$, namely where variable assignments are restricted to the set of representatives for each variable. Similarly, observe that the transition firings are as before, with the only difference that assignment updates associated to transitions are now restricted as well, or more precisely only the representatives are used: 
%%
\[
\restrict{\varState}'(\var) = \left\{\begin{array}{lr}
\restrict{\varState}(\var) & \text{if} \; \varname\not\in \writes(t),\\
rep(w(\var)) & \text{otherwise}.\\
\end{array}\right.
\]

This means that two legal firings $(M,\varState) \goto{t,w_1} (M,\varState_1)$ and $(M,\varState) \goto{t,w_2} (M,\varState_2)$ in the original (canonical) DPN-net $N$ correspond in $N_{\Repres{}}$ to the same firing $(M,\restrict{\varState}) \goto{t,w} (M,\restrict{\varState}')$ iff $w(\varname)=rep(w_1(\varname))=rep(w_2(\varname))$ for every $\varname\in \writes(t)$, which also implies that $\restrict{\varState}'$ is the restriction of both $\varState_1$ and $\varState_2$ with respect to $\Repres{}$.

\paolo{ho cercato in tutti i modi di definire quanto sotto rispetto anche agli assignment e quindi alle possibili guardie che si possono scrivere (dicendo quindi che soddisfano gli stessi test), ma diventa un vero casino. Ora dice solo che posso fare le stesse sequenze di t e raggiungere gli stessi marking.}

\begin{definition}[Run equivalence]
We say that a run $(M_I,\varState^0_1) \xrightarrow{\sigma_1} (M_1^n,\varState_1^n)$ of $N_1$ and a run $(M_I,\varState_2^0) \xrightarrow{\sigma_2} (M_2^n,\varState_2^n)$ of $N_2$ are \emph{equivalent} iff $M^0_1=M^0_2$ and for any $i\in [1,n]$ we have that $t^i_1=t^i_2$, $M^i_1=M^i_2$. 
 \end{definition}

Note that the definition above does not state a relation between each $\varState^i_1$ and $\varState^i_2$, although their existence follows.

\paolo{visto che la semantica, dato ogni (t,w), e' deterministica, allora trace equivalence e' uguale a simulation equivalence sul reachability graph e quindi sulle run. Tuttavia ho definito l'equivalenza come una proprieta' definita ricorsiva sulle run, anche se non serve davvero, perche' mi sembra piu convincente.}

Given two DPN-nets $N_1$ and $N_2$, we say that they are \emph{equivalent}  iff for every legal run $\rho_1$ of $N_1$ there exists an equivalent run $\rho_2$ of $N_2$ so that for any legal transition firing $\rho_1 \goto{t_1^{n+1},w_1^{n+1}} (M_1^{t+1},\varState_1^{t+1})$ there exists a run $\rho_2 \goto{t_2^{n+1},w_2^{n+1}} (M_2^{t+1},\varState_2^{t+1})$ that is equivalent. And vice-versa.

\begin{proposition}
Given a DPN-net $N$, $N$ is \emph{equivalent} to $N_{\Repres{}}$.
\end{proposition}


The intuition behind this proposition is that for any possible \emph{legal} process trace $\sigma = \tup{(t^1,w^1),\ldots, (t^n,w^n)}$ of $N$ we replace the run: 
\begin{equation}
(M_I,\varState_I) \xrightarrow{t^1,w^1} (M^1,\varState^1) \xrightarrow{t^2,w^2} \ldots \xrightarrow{t^n,w^n} (M^n,\varState^n) \text{ of } N \text{ by}
\label{eq1}
\end{equation}
\begin{equation}
(M_I,\restrict{\varState_I}) \xrightarrow{t^1,w^1} (M^1,\restrict{\varState}^1) \xrightarrow{t^2,w^2} \ldots \xrightarrow{t^n,w^n} (M^n,\restrict{\varState}^n) \text{ of } N_{\Repres{}},
\label{eq2}
\end{equation}

\noindent
where $\restrict{\varState}^i$ is the restriction of $\varState^i$ with respect to $\Repres{}$, for each $i\in[1,n]$.

\begin{proof}
First, observe that the claim holds for runs of length $0$.  Then, assume a legal trace $\sigma\in \dpnLang(N)$ and a legal trace $\restrict{\sigma}$ in $\dpnLang(N_{\Repres{}})$ of length $j-1\geq 0$, so that the corresponding runs are equivalent. 
%%
Towards contradiction, assume the claim is not true for $j$. 

$(\Rightarrow)$ Given a legal trace $\sigma\in \dpnLang(N)$ of length $j$ and its corresponding run as in (\ref{eq1}), if the run as in (\ref{eq2}) is not a run of $N_{\Repres{}}$ or it is not equivalent, then either $(a)$ $\restrict{\varState}^i$ cannot be defined (it is not possible to select a representative) or $(b)$ $(M^j,\restrict{\varState}^j) \xrightarrow{t^j,w^j} (M^{j+1},\restrict{\varState}^{j+1})$ is not legal. If $(a)$ is true then there exists a variable $\var\in\Vars$ such that $\varState^j(\var)=x$ but $x\not\in\Repres{\var}$. By definition, this means that $x\not\in\Consts{\var}$ and there are no two consecutive $x_1,x_2\in\Consts{\var}$ with $x\in(x_1,x_2)$. This is only possible if the open interval $(x_1,x_2)$ is empty (for instance, due to the fact that the domain is not dense), but this contradicts the fact that $\varState^j(\var)=x$. Regarding $(b)$, the transition firing is not legal, by definition iff, considering $\guard(t^j)=(\phi,\phi')$, then  $(b1)$ we have $\phi_{[\restrict{\varState}^j]}$ is not satisfied; $(b2)$ ${\phi'}_{[\restrict{\varState'}^j]}$ is not satisfied; $(b3)$ $t$ cannot fire or it is not true that $M^{j-1} [ t^j \rangle M^j$. If $(b1)$ is true it means that for some $\var\in\Vars$ either $\phi=\var$ and $\restrict{\varState}^j(\var)=\bot$ or $\phi$ is of the form $\var\odot k$ but it is not the case that $\odot(x,k)$ for $x=\restrict{\varState}^j(\var)$. In the former case  $\varState^j(\var)=\bot$ and $\phi_{[\varState^j]}\neq\true$ as well, while the latter is not possible either: if $x$ is a constant in $\Consts{\var}$ then it must be $\phi_{[\varState^j]}\neq\true$, whereas if it is a representative $x\in(x_1,x_2)$ then there must exist another constant in $\Consts{\var}\in(x_1,x_2)$, which implies that these are not consecutive constants. If case ($b2$) is true then either $w^j$ is not legal or the same reasoning as the previous case applies. Finally, if ($b3$) is true then $\sigma$ is not legal.
%%

$(\Leftarrow)$  Given a legal run $\restrict{\sigma}\in \dpnLang(N_{\Repres{}})$ of length $j$, if the corresponding run as in (\ref{eq1}) is not a run in $\dpnLang(N)$ or it is not equivalent to (\ref{eq1}), then either $(a)$ for some variable $\Vars$ there is no variable assignment $\varState^j(\var)$ with restriction $\restrict{\varState}^j$ or $(b)$ $(M^{j-1},\restrict{\varState}^{j-1}) \xrightarrow{t^j,w^j} (M^j,\restrict{\varState}^j)$ is not legal given the guards $(\phi,\phi')=\guard(t^j)$. Case $(a)$ is not possible by definition of the representative net, whereas if $(b)$ is true then either $(b1)$ $\phi_{[\varState^j]}\neq\true$ for any $\varState^j$ as before, or $(b2)$ the same holds for $\phi'_{[\varState'^j]}$, or $(b3)$ $t^j$ cannot fire or  it is not true that $M^{j-1} [ t^j \rangle M^j$. If $(b1)$ then for some variable $\var$ either $\phi=\var$ and $\restrict{\varState}^j(\var)=\bot$ or $\phi=\var\odot k$ but $\phi_{[\varState^j]}$ for every possible value $x$ so that $rep(x)=\restrict{\varState}^j(\var)$. Both cases are clearly not possible unless $\phi_{[\restrict{\varState}^j]}\neq\true$. The same reasoning applies for $(b2)$, while $(b3)$ falsifies the assumption that $\restrict{\sigma}$ is legal.  
\end{proof}

As a corollary, any property as in Definition~\ref{def:properties} holds in $N$ iff it holds in $N_{\Repres{}}$. 
